Extreme Rotation Estimation in the Wild

We present a technique and benchmark dataset for estimating the relative 3D orientation between a pair of Internet images captured in an extreme setting, where the images have limited or non-overlapping field of views. Prior work targeting extreme rotation estimation assume constrained 3D environments and emulate perspective images by cropping regions from panoramic views. However, real images captured in the wild are highly diverse, exhibiting variation in both appearance and camera intrinsics. In this work, we propose a Transformer-based method for estimating relative rotations in extreme real-world settings, and contribute the ExtremeLandmarkPairs dataset, assembled from scene-level Internet photo collections. Our evaluation demonstrates that our approach succeeds in estimating the relative rotations in a wide variety of extreme-view Internet image pairs, outperforming various baselines, including dedicated rotation estimation techniques and contemporary 3D reconstruction methods.

==> tables/10_fov_diff.tex <==
\definecolor{graytext}{RGB}{130,130,130}
\begin{table}[t]
\setlength{\tabcolsep}{1.7pt}
% \def\arraystretch{1.05}
 \def\arraystretch{1}
%  \footnotesize
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{llcccccccccc} %{0.88\textwidth}

    \toprule
    \multicolumn{2}{c}{}&&\multicolumn{3}{c}{\cambridge{}}&&
    \multicolumn{3}{c}{\megadepth{}}\\
    \cline{4-6} \cline{8-10}
      & Method &&MGE\textdownarrow & RRA$_{15}$\textuparrow &RRA$_{30}$\textuparrow && MGE\textdownarrow & RRA$_{15}$ \textuparrow & RRA$_{30}$\textuparrow \\
    \midrule

    \multirow{2}{*}{\rotatebox[origin=c]{90}{Large}} & 
    $\Delta5^\circ$ &&   2.45 & 96.7 & 96.8 &&   {2.41}  & {97.5}  & {97.9}  \\
    & $\Delta10^\circ$ &&   2.42 & 98.3 & 98.4 &&   {2.40}  & 97.9  & {98.2}  \\
    \midrule
   \multirow{2}{*}{\rotatebox[origin=c]{90}{Small}} &
   $\Delta5^\circ$  &&   4.35 & 88.3 & 89.0 &&  {4.47} &  {87.2} & {91.6} \\
   & $\Delta10^\circ$ &&   4.17 & 88.4 & 89.2 &&  {4.66} &  {89.0} & {93.1} \\
   \midrule
   \multirow{2}{*}{\rotatebox[origin=c]{90}{None}} & 
   $\Delta5^\circ$ &&   13.62 & 52.7 & 59.7 && 26.97 & 36.1 & 50.7 \\
   & $\Delta10^\circ$ &&   14.70 & 50.6 & 58.6 && 33.46 & 34.8 & 48.8 \\
    \bottomrule
\end{tabular}
}
\caption{Ablation study, evaluating the effect of FoV difference threshold }
%}

\label{tab:10_fov_diff}
\end{table}


==> tables/The_effect_of_auxillary_channels.tex <==
\definecolor{graytext}{RGB}{130,130,130}
\begin{table}[t]
\setlength{\tabcolsep}{1.7pt}
% \def\arraystretch{1.05}
 \def\arraystretch{1.2}
%  \footnotesize
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lllccccccccccccccccc} %{0.88\textwidth}
%{p{1.5cm}p{1.5cm}p{1.5cm}lp{1.5cm}p{1.5cm}p{1.5cm}lp{1.5cm}p{1.5cm}p{1.5cm}}
    \toprule
    & & \multicolumn{3}{c}{}&\multicolumn{3}{c}{Top 1} & & \multicolumn{3}{c}{Top 5} \\
     \cline{6-8} \cline{10-12}
     &Overlap & KP & SM &&MGE & RRA$_{15}$ &RRA$_{30}$ && MGE & RRA$_{15}$ & RRA$_{30}$ \\
    \midrule
    % Add your data rows here
    %TODO - instruct w removed scenes
     %\hline
%      \multirow{9}{*}{\rotatebox[origin=c]{90}{\cambridge{}} } & {Large} &  $\times$ & \checkmark && 2.56  & \underline{97.0}  & \underline{97.1}  && 2.59  & \underline{98.6}  & \underline{99.6}  \\
%      & & \checkmark & $\times$ && \underline{2.43}  & \textbf{99.6}  & \textbf{99.7}  && \underline{2.42}  & \textbf{99.7}  & \textbf{100.0}  \\
%    %\cline{3-11}
%    & & \checkmark & \checkmark && \textbf{2.35} & 96.5 & 96.5 && \textbf{2.36} & 96.6 & 96.7 \\
%    %\cline{2-11}
%    &{Small} & $\times$ & \checkmark && \underline{4.42}  & 87.7  &  \underline{90.1} && \underline{4.29}  & \underline{91.9}  & \underline{96.0}  \\
%    && \checkmark & $\times$ && \textbf{4.18}  & \textbf{91.7}  & \textbf{93.6}  && \textbf{4.13}  & \textbf{95.9}  & \textbf{98.9}  \\
%    %\cline{3-11}
%    & & \checkmark & \checkmark && 4.44 & \underline{88.5} & 89.6 && 4.35 & 91.8 & 94.1 \\
%    %\cline{2-11}
%    &{None} & $\times$ & \checkmark && 15.74 & 48.5  & 57.9  && 10.28  & 70.8  & 90.7  \\
%    && \checkmark & $\times$ && \underline{13.53}  &  \textbf{53.5}  & \textbf{63.6}  && \underline{9.26}  & \textbf{77.7}  & \textbf{95.6} \\
%    & & \checkmark & \checkmark && \textbf{13.36} & \underline{52.9} & \underline{59.7} && \textbf{9.17} & \underline{76.6} & \underline{94.5} \\
%    \hline
    
%   \multirow{9}{*}{\rotatebox[origin=c]{90}{\megadepth{} }}
%   & {Large}  & $\times$ & \checkmark && 2.57  & 96.3  & 97.0  && 2.57  & 98.2  & \underline{99.6}  \\
%   %\cline{3-11}
%   && \checkmark & $\times$ && \textbf{2.39} & \textbf{97.7}  & \textbf{98.4} 
%   && \textbf{2.34}  & \underline{98.5}  & \textbf{99.7} \\
%   %\cline{3-11}
%   & & \checkmark & \checkmark && \underline{2.40}  & \textbf{97.7}  & \underline{98.2}  && \underline{2.39}  & \textbf{98.6}  & 99.4 \\
%   %\cline{2-11}
%   &{Small} & $\times$ & \checkmark && 5.57  & 81.4  & 88.8  && 5.28  & 87.1  & 96.0  \\
%   & & \checkmark & $\times$ && \underline{4.75} &\underline{ 84.0}  & \underline{89.4}   && \underline{4.53}  & \underline{89.1}  & \underline{96.5} \\
%   %\cline{3-11}
%   & & \checkmark & \checkmark && \textbf{4.33} & \textbf{88.1} & \textbf{92.3} && \textbf{4.12} & \textbf{91.2} & \textbf{97.1}  \\
%   %\cline{2-11}
%   &{None} & $\times$ & \checkmark && 46.0  & 28.5  & 42.5  && 14.75  & 50.7  & 79.2  \\ 
%   && \checkmark & $\times$ && \underline{42.09} & \underline{33.4}  & \underline{45.9}  
%   && \underline{12.78}  & \underline{56.3}  & \underline{84.0}  \\
%   & & \checkmark & \checkmark &&  \textbf{27.49} & \textbf{36.2} & \textbf{50.5} && \textbf{13.03} & \textbf{57.1} & \textbf{85.1}  \\
%
    \multirow{9}{*}{\rotatebox[origin=c]{90}{\cambridge{}} } & {Large} & $\times$ & $\times$ && 2.24  & 92.8  & 93.2  && 2.24  & 98.3  & 98.9  \\ 
    &&  $\times$ & \checkmark && 2.56  & 97.0  & 97.1  && 2.59  & 98.6  & 99.6  \\
      & & \checkmark & $\times$ && 2.43  &  \textbf{99.6}  &  \textbf{99.7}  && 2.42  &  \textbf{99.7}  &  \textbf{100.0}  \\
    %\cline{3-11}
    & & \checkmark & \checkmark &&  \textbf{2.35} & 96.5 & 96.5 &&  \textbf{2.36} & 96.6 & 96.7 \\
    %\cline{2-11}
    &{Small} & $\times$ & $\times$ && 4.31  & 91.7  & 93.3  && 4.28  & 94.8  & 98.2  \\ 
    && $\times$ & \checkmark && 4.42  & 87.7  &  90.1 && 4.29  & 91.9  & 96.0  \\
    && \checkmark & $\times$ &&  \textbf{4.18} &  \textbf{91.7}  &  \textbf{93.6} &&  \textbf{4.13}  &  \textbf{95.9}  &  \textbf{98.9}  \\
    %\cline{3-11}
    & & \checkmark & \checkmark && 4.44 & 88.5 & 89.6 && 4.35 & 91.8 & 94.1 \\
    %\cline{2-11}
    &{None} & $\times$ & $\times$ && 20.44  & 45.0  & 53.1  && 10.05  & 68.5  & 87.2  \\ 
    && $\times$ & \checkmark && 15.74 & 48.5  & 57.9  && 10.28  & 70.8  & 90.7  \\
    && \checkmark & $\times$ && 13.53  &   \textbf{53.5}  &  \textbf{63.6}  && 9.26  &  \textbf{77.7}  &  \textbf{95.6} \\
    & & \checkmark & \checkmark &&  \textbf{13.36} & 52.9 & 59.7 &&  \textbf{9.17} & 76.6 & 94.5 \\
    \hline
    
    \multirow{9}{*}{\rotatebox[origin=c]{90}{\megadepth{} }}
    & {Large}  & $\times$ & $\times$ && 2.19  & 96.0  & 96.6  && 2.23  & 98.3  & 99.3  \\ 
    && $\times$ & \checkmark && 2.57  & 96.3  & 97.0  && 2.57  & 98.2  & 99.6  \\
    %\cline{3-11}
    && \checkmark & $\times$ &&  \textbf{2.39} & 97.7  &  \textbf{98.4} 
    &&  \textbf{2.34}  &  98.5  &  \textbf{99.7} \\
    %\cline{3-11}
    & & \checkmark & \checkmark && 2.40  &  \textbf{97.7}  & 98.2  && 2.39 &  \textbf{98.6}  & 99.4 \\
    %\cline{2-11}
    &{Small} & $\times$ & $\times$ && 4.39  & 87.8  & 91.2  && 4.24  & 91.0  & 95.2  \\ 
    && $\times$ & \checkmark && 5.57  & 81.4  & 88.8  && 5.28  & 87.1  & 96.0  \\
    & & \checkmark & $\times$ && 4.75 & 84.0  & 89.4   && 4.53  & 89.1  & 96.5 \\
    %\cline{3-11}
    & & \checkmark & \checkmark &&  \textbf{4.33} &  \textbf{88.1} &  \textbf{92.3} &&  \textbf{4.12} &  \textbf{91.2} &  \textbf{97.1}  \\
    %\cline{2-11}
    &{None} 
    & $\times$ & $\times$ && 49.31  & 33.1  & 44.0  && 12.92  & 56.5  &  \textbf{85.4}  \\ 
    && $\times$ & \checkmark && 46.00  & 28.5  & 42.50  && 14.75  & 50.7  & 79.2  \\ 
    && \checkmark & $\times$ && 42.09 & 33.4  & 45.9  
    && \textbf{12.78}  & 56.3  & 84.0  \\
    & & \checkmark & \checkmark &&   \textbf{27.49} &  \textbf{36.2} &  \textbf{50.5} &&  13.03 &  \textbf{57.1} &  {85.1}  \\
    \bottomrule
\end{tabular}
}
\caption{Ablation study, evaluating the effect of the auxiliary channels added as input to our network. We train models without the keypoints and matches (KP) and without the segmentation maps (SM), and compare with our full model that is provided with both.} %\hec{add two x's} }
\label{tab:auxillary_long}
\end{table}

==> tables/The_effect_of_our_data_augmentations.tex <==
\definecolor{graytext}{RGB}{130,130,130}
\begin{table}[t]
\setlength{\tabcolsep}{1.7pt}
% \def\arraystretch{1.05}
 \def\arraystretch{1.2}
%  \footnotesize
\centering
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{llccccccccccccccccc} %{0.88\textwidth}
    \toprule
    & & && &&\multicolumn{3}{c}{Top 1} & & \multicolumn{3}{c}{Top 5} \\
     \cline{7-9} \cline{11-13}
     &Overlap  & \cite{cai2021extreme} & \fovexp{} & \instructexp{} && MGE & RRA$_{15}$ &RRA$_{30}$ && MGE & RRA$_{15}$ & RRA$_{30}$ \\
    \midrule
    % Add your data rows here
     %\hline
%      \multirow{12}{*}{\rotatebox[origin=c]{90}{\cambridge{}} } & {Large} & $\times$&$\times$& $\times$ && 11.52  & 63.9  & 96.3  && 11.34  & 66.0  & 97.6  \\
%    %\cline{3-11}
%    & & \checkmark&$\times$& $\times$ && 2.82  & \textbf{99.2}  & \textbf{99.6}  && 2.72  & \textbf{99.4}  & \textbf{99.8}  \\
%    %\cline{3-11}
%    %& & $\vee$&$\vee$&$\vee$ && 2.91  & \textbf{99.8}  & \textbf{99.8}  && 2.87  & \textbf{99.8}  & \textbf{100.0}  \\
%    & & \checkmark&\checkmark& $\times$ && \textbf{2.35}  & \underline{96.3}  & \underline{96.5}  && \textbf{2.36}  & \underline{96.5}  & \underline{96.8}  \\
%    %\cline{3-11}
%    &  & \checkmark& \checkmark& \checkmark && \underline{2.37} & 95.8 & 95.8 && \underline{2.37} & 95.9 & 96.1\\
%    %\cline{2-11}
%    &{Small} & $\times$&$\times$& $\times$ && 40.16  & 16.4  & 32.2  && 20.07  & 37.8  & 64.6 \\
%    %\cline{3-11}
%
%    & & \checkmark &$\times$& $\times$ && 5.88  & 84.9  & \textbf{91.4}  && 5.51  & 89.6  & \textbf{97.1}  \\
%    %& & $\vee$&$\vee$&$\vee$&& 5.87  & \textbf{89.4}  & \textbf{93.2}  && 5.47  & \textbf{93.0}  & \textbf{99.5}  \\
%    & & \checkmark & \checkmark& $\times$ && \textbf{4.25}  & \textbf{89.0}  & \underline{90.0}  && \textbf{4.17}  & \textbf{92.7}  & \underline{94.9}  \\
%    %\cline{3-11}
%    & & \checkmark & \checkmark& \checkmark && \underline{4.5} & \underline{88.2} & 89.3 && \underline{4.38} & \textbf{92.7} & 94.6  \\
%    %\cline{2-11}
%    &{None}& $\times$&$\times$& $\times$ && 86.87  & 6.5  & 15.2  && 24.53  & 32.4  & 59.9  \\
%    %\cline{3-11}
%    & & \checkmark &$\times$& $\times$ && 19.00  & 43.8  & 56.3  && 10.72  & 67.8  & 88.0  \\
%    %\cline{3-11}
%    %& & $\vee$&$\vee$&$\vee$&& 16.40  & 47.9  & 59.5  && 10.23  & 70.7  & 93.5  \\
%     & & \checkmark & \checkmark& $\times$ && \underline{13.77}  & \underline{52.5}  & \textbf{60.3}  && \underline{9.21}  & \underline{76.5}  & \textbf{94.8}  \\
%    %\cline{3-11}
%    &  & \checkmark & \checkmark& \checkmark && \textbf{13.27} & \textbf{52.7} & \underline{59.9} &&  \textbf{9.17} & \textbf{76.9} & \underline{94.0} \\
%    \midrule
%    \multirow{12}{*}{\rotatebox[origin=c]{90}{\megadepth{} }}
% & {Large} & $\times$ & $\times$& $\times$ && 10.21  & 69.8  & 95.1  && 9.83  & 73.8  & 97.9  \\
    %\cline{3-11}
%    & & \checkmark & $\times$ & $\times$ && 2.96  & 96.0  & 97.3  && 2.88  & 96.9  & 98.5  \\
%    %\cline{3-11}
%    %& & $\vee$&$\vee$&$\vee$&& 2.67  & 96.9  & \underline{98.0}  && 2.62 & 98.2  & \textbf{99.7}  \\
%    & & \checkmark & \checkmark& $\times$ && \textbf{2.39}  & \underline{97.6}  & \underline{98.0}  && \underline{2.40}  & \textbf{98.7}  & \textbf{99.6}  \\
%    %\cline{3-11}
%    &  & \checkmark & \checkmark& \checkmark && \underline{2.40}  & \textbf{97.7}  & \textbf{98.2}  && \textbf{2.39}  & \underline{98.6}  & \underline{99.4} \\
%    
%    %\cline{2-11}
%    &{Small} & $\times$ & $\times$ & $\times$ && 30.22 & 19.9  & 48.9  
%    && 15.75  & 48.5  & 79.1 \\
%    %\cline{3-11}
%    & & \checkmark & $\times$ & $\times$ && 8.03  & 71.8  & 85.5  && 6.95  & 78.6  & 93.2  \\
%    %& & $\vee$&$\vee$&$\vee$&& 6.35  & 80.9  & 90.0  && 6.09  & 87.1  & \textbf{97.9}  \\
%    %\cline{3-11}
%    & & \checkmark & \checkmark& $\times$ && \underline{4.56}  & \underline{86.6}  & \underline{91.3}  && \underline{4.46}  & \underline{90.7}  & \textbf{97.2}  \\
%    %\cline{3-11}
%    &  & \checkmark & \checkmark& \checkmark && \textbf{4.33} & \textbf{88.1} & \textbf{92.3} && \textbf{4.12} & \textbf{91.2} & \underline{97.1}  \\
%    %\cline{2-11}
%    &{None} & $\times$&$\times$& $\times$ && 70.68 & 7.9  & 22.9  
%    && 23.63  & 28.1  & 62.8 \\
%    %\cline{3-11}
%    &&  \checkmark & $\times$ & $\times$ && 44.66  & 27.2  & 42.0  && 14.96  & 50.4  & 83.4  \\
%    %\cline{3-11}
%    %& & $\vee$&$\vee$&$\vee$ && 66.87  & 26.1  & 36.2  && 15.53  & 47.3  & 75.0  \\
%    &  & \checkmark & \checkmark& $\times$ && \underline{30.66}  & \underline{35.6}  & \underline{49.9}  && \underline{13.25}  & \underline{56.3}  & \textbf{85.2}  \\
%    %\cline{3-11}
%    &  & \checkmark & \checkmark& \checkmark &&   \textbf{27.49} & \textbf{36.2} & \textbf{50.5} && \textbf{13.03} & \textbf{57.1} & \underline{85.1}  \\


    \multirow{12}{*}{\rotatebox[origin=c]{90}{\cambridge{}} } & {Large} & $\times$&$\times$& $\times$ && 11.52  & 63.9  & 96.3  && 11.34  & 66.0  & 97.6  \\
    %\cline{3-11}
    & & \checkmark&$\times$& $\times$ && 2.82  &  \textbf{99.2}  &  \textbf{99.6}  && 2.72  &  \textbf{99.4}  &  \textbf{99.8}  \\
    %\cline{3-11}
    %& & $\vee$&$\vee$&$\vee$ && 2.91  & \textbf{99.8}  & \textbf{99.8}  && 2.87  & \textbf{99.8}  & \textbf{100.0}  \\
    & & \checkmark&\checkmark& $\times$ &&  \textbf{2.35} & 96.3  & 96.5  &&  \textbf{2.36} & 96.5  & 96.8  \\
    %\cline{3-11}
    &  & \checkmark& \checkmark& \checkmark && 2.37 & 95.8 & 95.8 && 2.37 & 95.9 & 96.1\\
    %\cline{2-11}
    &{Small} & $\times$&$\times$& $\times$ && 40.16  & 16.4  & 32.2  && 20.07  & 37.8  & 64.6 \\
    %\cline{3-11}

    & & \checkmark &$\times$& $\times$ && 5.88  & 84.9  & 91.4  && 5.51  & 89.6  & 97.1  \\
    %& & $\vee$&$\vee$&$\vee$&& 5.87  & \textbf{89.4}  & \textbf{93.2}  && 5.47  & \textbf{93.0}  & \textbf{99.5}  \\
    & & \checkmark & \checkmark& $\times$ &&  \textbf{4.25}  &  \textbf{89.0}  &  \textbf{90.0}  &&  \textbf{4.17}  &  \textbf{92.7}  &  \textbf{94.9}  \\
    %\cline{3-11}
    & & \checkmark & \checkmark& \checkmark && 4.5 & 88.2 & 89.3 && 4.38 &  \textbf{92.7} & 94.6  \\
    %\cline{2-11}
    &{None}& $\times$&$\times$& $\times$ && 86.87  & 6.5  & 15.2  && 24.53  & 32.4  & 59.9  \\
    %\cline{3-11}
    & & \checkmark &$\times$& $\times$ && 19.00  & 43.8  & 56.3  && 10.72  & 67.8  & 88.0  \\
    %\cline{3-11}
    %& & $\vee$&$\vee$&$\vee$&& 16.40  & 47.9  & 59.5  && 10.23  & 70.7  & 93.5  \\
     & & \checkmark & \checkmark& $\times$ && 13.77  & 52.5  &  \textbf{60.3}  && 9.21  & 76.5  &  \textbf{94.8}  \\
    %\cline{3-11}
    &  & \checkmark & \checkmark& \checkmark &&  \textbf{13.27} &  \textbf{52.7} & 59.9 &&   \textbf{9.17} &  \textbf{76.9} & 94.0 \\
    \midrule
    \multirow{12}{*}{\rotatebox[origin=c]{90}{\megadepth{} }}
 & {Large} & $\times$ & $\times$& $\times$ && 10.21  & 69.8  & 95.1  && 9.83  & 73.8  & 97.9  \\
    %\cline{3-11}
    & & \checkmark & $\times$ & $\times$ && 2.96  & 96.0  & 97.3  && 2.88  & 96.9  & 98.5  \\
    %\cline{3-11}
    %& & $\vee$&$\vee$&$\vee$&& 2.67  & 96.9  & \underline{98.0}  && 2.62 & 98.2  & \textbf{99.7}  \\
   & & \checkmark & \checkmark& $\times$ && \textbf{ 2.39}  & 97.6  & 98.0  && 2.40  &  \textbf{98.7}  &  \textbf{99.6}  \\
    %\cline{3-11}
    &  & \checkmark & \checkmark& \checkmark && 2.40  &  \textbf{97.7}  &  \textbf{98.2}  &&  \textbf{2.39} & 98.6  & 99.4 \\
    
    %\cline{2-11}
    &{Small} & $\times$ & $\times$ & $\times$ && 30.22 & 19.9  & 48.9  
    && 15.75  & 48.5  & 79.1 \\
    %\cline{3-11}
    & & \checkmark & $\times$ & $\times$ && 8.03  & 71.8  & 85.5  && 6.95  & 78.6  & 93.2  \\
    %& & $\vee$&$\vee$&$\vee$&& 6.35  & 80.9  & 90.0  && 6.09  & 87.1  & \textbf{97.9}  \\
    %\cline{3-11}
    & & \checkmark & \checkmark& $\times$ && 4.56  & 86.6  & 91.3  && 4.46  & 90.7  & 97.2  \\
    %\cline{3-11}
    &  & \checkmark & \checkmark& \checkmark &&  \textbf{4.33} &  \textbf{88.1} &  \textbf{92.3} &&  \textbf{4.12} &  \textbf{91.2} &  \textbf{97.1}  \\
    %\cline{2-11}
    &{None} & $\times$&$\times$& $\times$ && 70.68 & 7.9  & 22.9  
    && 23.63  & 28.1  & 62.8 \\
    %\cline{3-11}
    &&  \checkmark & $\times$ & $\times$ && 44.66  & 27.2  & 42.0  && 14.96  & 50.4  & 83.4  \\
    %\cline{3-11}
    %& & $\vee$&$\vee$&$\vee$ && 66.87  & 26.1  & 36.2  && 15.53  & 47.3  & 75.0  \\
    &  & \checkmark & \checkmark& $\times$ && 30.66  & 35.6  & 49.9  && 13.25  & 56.3  & 85.2  \\
    %\cline{3-11}
    &  & \checkmark & \checkmark& \checkmark &&    \textbf{27.49} &  \textbf{36.2} &  \textbf{50.5} &&  \textbf{13.03} &  \textbf{57.1} &  \textbf{85.1}  \\
    \bottomrule
\end{tabular}
}
\caption{We evaluate to what extent the progressive training scheme is needed, in contrast to simply training on real image pairs. In the first rows (three $\times$'s), we train models on \dataset{} \emph{only}. In the rows below, we first train on the panoramas, according to our progressive training scheme. As illustrated above, training on panoramas, along with the various data augmentations we propose, significantly improve performance, particularly for non-overlapping image pairs. } 
\label{tab:data_aug}
\end{table}

==> tables/ablation.tex <==
\definecolor{graytext}{RGB}{130,130,130}
\begin{table}[t]
\setlength{\tabcolsep}{1.7pt}
% \def\arraystretch{1.05}
 \def\arraystretch{1.2}
%  \footnotesize
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lllccccccccccccccccc} %{0.88\textwidth}
%{p{1.5cm}p{1.5cm}p{1.5cm}lp{1.5cm}p{1.5cm}p{1.5cm}lp{1.5cm}p{1.5cm}p{1.5cm}}
    \toprule
    & \multicolumn{3}{c}{}&\multicolumn{3}{c}{Top 1} & & \multicolumn{3}{c}{Top 5} \\
     \cline{5-7} \cline{9-11}
     &Overlap & Train data &&MGE & RRA$_{15}$ &RRA$_{30}$ && MGE & RRA$_{15}$ & RRA$_{30}$ \\
    \midrule
    % Add your data rows here
    %TODO - instruct w removed scenes
     %\hline
%    \multirow{12}{*}{\rotatebox[origin=c]{90}{\cambridge{}} } & Large & \cite{cai2021extreme} &&  8.17 & 86.4 & 97.1 && 8.17 & 87.5 & 98.1\\
% % \cline{3-11}
%  & & +\fovexp{} && \underline{3.18} & \underline{98.2} & \underline{98.2} && \underline{3.21} & \underline{97.9}& \underline{98.7} \\
% % \cline{3-11}
%  & & +\instructexp{} && 3.10 & \textbf{99.4} & \textbf{99.5} && 4.04 & \textbf{98.5} & \textbf{98.9} \\
% % \cline{3-11}
%  %& & +\shortdataset{} && \textbf{2.32} & 89.9 & 89.9 && \textbf{2.31} & 89.9 & 90.2  & \vspace{1pt} \\ 
%  & & +\shortdataset{} && \textbf{2.35} & 96.5 & 96.5 && \textbf{2.36} & 96.6 & 96.7  & \vspace{1pt} \\ 
%%  \cline{2-11}
%  &Small & \cite{cai2021extreme} && 26.44 & 6.3 & 60.2 && 22.32 & 17.4 & 69.5\\
%%  \cline{3-11}
%  & & +\fovexp{} && \underline{5.14} & 79.8 & 82.6 && \underline{5.24} & 85.5 & 92.1 \\
% % \cline{3-11}
%   & & +\instructexp{} && 5.91 & \underline{83.9} & \underline{88.4} && 5.84 & \underline{88.3} & \textbf{95.5} \\
% % \cline{3-11}
%  %& & +\shortdataset{} && \textbf{4.53} & \underline{82.8} & \underline{85.5} && \textbf{4.36} & \underline{86.3} & 90.9  & \vspace{1pt} \\
 %   & & +\shortdataset{} && \textbf{4.44} & \textbf{88.5} & \textbf{89.6} && \textbf{4.35} & \textbf{91.8} & \underline{94.1}  & \vspace{1pt} \\
 % %  \cline{2-11}
 %   &None & \cite{cai2021extreme} && 76.63 & 17.9 & 32.9 && 17.54 & 42.0 & 78.9 \\
 % %  \cline{3-11}
 %   & & +\fovexp{} && 28.22 & 42.4 & 49.7 && 10.52 & 71.0 & 90.8 \\
 % %  \cline{3-11}
 %   & & +\instructexp{} && \underline{14.20} & \underline{50.1} & \underline{60.1} && \underline{9.76} & \underline{72.7} & \underline{92.6} \\
 %   %\cline{3-11}
 %    %& & +\shortdataset{} && \textbf{13.29} & \textbf{51.7} & \underline{57.1} && \textbf{9.28} & \textbf{72.8} & 90.2 \\
 %    & & +\shortdataset{} && \textbf{13.36} & \textbf{52.9} & \textbf{59.7} && \textbf{9.17} & \textbf{76.6} & \textbf{94.5} \\
 %   \midrule
 %    \multirow{12}{*}{{\rotatebox[origin=c]{90}\megadepth{}}} & Large & \cite{cai2021extreme} && 13.65 & 35.4 & 73.5 && 12.22 & 61.4 & 84.7\\
 %   %\cline{3-11}
 %   & & +\fovexp{} && 4.61 & 79.7 & 81.1 && \underline{4.41} & 90.3& 98.9\\
 %   %\cline{3-11}
 %   & & +\instructexp{} && \underline{4.46} & \underline{90.4} & \underline{92.4} && 4.43 & \underline{94.3} & \underline{99.1} \\
    %\cline{3-11}
    %& & +\shortdataset{} && \textbf{2.21} & \textbf{97.4} & \textbf{98.2} && \textbf{2.19} & \textbf{98.0} & \textbf{99.1} & \vspace{1pt}\\
%    & & +\shortdataset{} && \textbf{2.40} & \textbf{97.7} & \textbf{98.2} && \textbf{2.39} & \textbf{98.6} & \textbf{99.4} & \vspace{1pt}\\
%    %\cline{2-11}
%    &Small& \cite{cai2021extreme} && 55.28 & 3.7 & 29.1 && 29.83 & 15.0 & 50.3  \\
%    %\cline{3-11}
%    & & +\fovexp{} && 12.91 & 56.2 & 68.2 && 10.97 & 66.0 & 85.4 \\
%   % \cline{3-11}
%    & & +\instructexp{} && \underline{11.46} & \underline{62.5} & \underline{80.6} && \underline{10.73} & \underline{68.0} & \underline{91.0} \\
% %   \cline{3-11}
%     %& & +\shortdataset{} && \textbf{4.69} & \textbf{83.2} & \textbf{89.1} && \textbf{4.59} & \textbf{87.4} & \textbf{96.4} & \vspace{1pt}\\
%     & & +\shortdataset{} && \textbf{4.33} & \textbf{88.1} & \textbf{92.3} && \textbf{4.12} & \textbf{91.2} & \textbf{97.1} & \vspace{1pt}\\
%  %  \cline{2-11}
%    &None & \cite{cai2021extreme} && 74.94 & 12.8 & 25.3 && 25.11 & 26.1 & 58.8  \\
 %   \cline{3-11}
%    & & +\fovexp{} && \underline{61.62} & \underline{25.0} & \underline{38.4} && 16.82 & 44.2 & 75.0 \\
%    %\cline{3-11}
%    & & +\instructexp{} && 68.31 & \underline{25.0} & 36.1 && \underline{16.21} & \underline{45.7} & \underline{78.2} \\
%   % \cline{3-11}
      %& & +\shortdataset{} && \textbf{30.88} & \textbf{36.9} & \textbf{49.8} && \textbf{12.60} & \textbf{58.2} & \textbf{86.6} \\
%      & & +\shortdataset{} && \textbf{27.49} & \textbf{36.2} & \textbf{50.5} && \textbf{13.03} & \textbf{57.1} & \textbf{85.1} \\
      \multirow{12}{*}{\rotatebox[origin=c]{90}{\cambridge{}} } & Large &  \cite{cai2021extreme}&&  8.17 & 86.4 & 97.1 && 8.17 & 87.5 & 98.1\\
   % \cline{3-11}
    & & +\fovexp{}&& 3.18 & 98.2 & 98.2 && 3.21 & 97.9& 98.7 \\
   % \cline{3-11}
    & & +\instructexp{} && 3.10 & \textbf{99.4} & \textbf{99.5} && 4.04 & \textbf{98.5} & \textbf{98.9}\\
   % \cline{3-11}
    %& & +\shortdataset{} && \textbf{2.32} & 89.9 & 89.9 && \textbf{2.31} & 89.9 & 90.2  & \vspace{1pt} \\ 
    & & +\shortdataset{} && \textbf{2.35} & 96.5 & 96.5 && \textbf{2.36} & 96.6 & 96.7  & \vspace{1pt} \\ 
  %  \cline{2-11}
    &Small & \cite{cai2021extreme} && 26.44 & 6.3 & 60.2 && 22.32 & 17.4 & 69.5\\
  %  \cline{3-11}
    & & +\fovexp{} && 5.14 & 79.8 & 82.6 && 5.24 & 85.5 & 92.1 \\
   % \cline{3-11}
     & & +\instructexp{} && 5.91 & 83.9 & 88.4 && 5.84 & 88.3 & 95.5 \\
   % \cline{3-11}
    %& & +\shortdataset{} && \textbf{4.53} & \underline{82.8} & \underline{85.5} && \textbf{4.36} & \underline{86.3} & 90.9  & \vspace{1pt} \\
    & & +\shortdataset{} && \textbf{4.44} & \textbf{88.5} & \textbf{89.6} && \textbf{4.35} & \textbf{91.8} & \textbf{94.1}  & \vspace{1pt} \\
  %  \cline{2-11}
    &None & \cite{cai2021extreme} && 76.63 & 17.9 & 32.9 && 17.54 & 42.0 & 78.9 \\
  %  \cline{3-11}
    & & +\fovexp{} && 28.22 & 42.4 & 49.7 && 10.52 & 71.0 & 90.8 \\
  %  \cline{3-11}
    & & +\instructexp{} && 14.20 & 50.1 & 60.1 && 9.76 & 72.7 & 92.6 \\
    %\cline{3-11}
     %& & +\shortdataset{} && \textbf{13.29} & \textbf{51.7} & \underline{57.1} && \textbf{9.28} & \textbf{72.8} & 90.2 \\
     & & +\shortdataset{} && \textbf{13.36} & \textbf{52.9} & \textbf{59.7} && \textbf{9.17} & \textbf{76.6} & \textbf{94.5} \\
    \midrule
     \multirow{12}{*}{{\rotatebox[origin=c]{90}\megadepth{}}} & Large & \cite{cai2021extreme} && 13.65 & 35.4 & 73.5 && 12.22 & 61.4 & 84.7\\
    %\cline{3-11}
    & & +\fovexp{} && 4.61 & 79.7 & 81.1 && 4.41 & 90.3& 98.9\\
    %\cline{3-11}
    & & +\instructexp{} && 4.46 & 90.4 & 92.4 && 4.43 & 94.3 & 99.1 \\
    %\cline{3-11}
    %& & +\shortdataset{} && \textbf{2.21} & \textbf{97.4} & \textbf{98.2} && \textbf{2.19} & \textbf{98.0} & \textbf{99.1} & \vspace{1pt}\\
    & & +\shortdataset{} && \textbf{2.40} & \textbf{97.7} & \textbf{98.2} && \textbf{2.39} & \textbf{98.6} & \textbf{99.4} & \vspace{1pt}\\
    %\cline{2-11}
    &Small& \cite{cai2021extreme} && 55.28 & 3.7 & 29.1 && 29.83 & 15.0 & 50.3  \\
    %\cline{3-11}
    & & +\fovexp{} && 12.91 & 56.2 & 68.2 && 10.97 & 66.0 & 85.4 \\
   % \cline{3-11}
    & & +\instructexp{} && 11.46 & 62.5 & 80.6 && 10.73 & 68.0 & 91.0 \\
 %   \cline{3-11}
     %& & +\shortdataset{} && \textbf{4.69} & \textbf{83.2} & \textbf{89.1} && \textbf{4.59} & \textbf{87.4} & \textbf{96.4} & \vspace{1pt}\\
     & & +\shortdataset{} && \textbf{4.33} & \textbf{88.1} & \textbf{92.3} && \textbf{4.12} & \textbf{91.2} & \textbf{97.1} & \vspace{1pt}\\
  %  \cline{2-11}
    &None & \cite{cai2021extreme} && 74.94 & 12.8 & 25.3 && 25.11 & 26.1 & 58.8  \\
 %   \cline{3-11}
    & & +\fovexp{} && 61.62 & 25.0 & 38.4 && 16.82 & 44.2 & 75.0 \\
    %\cline{3-11}
    & & +\instructexp{} && 68.31 & 25.0 & 36.1 && 16.21 & 45.7 & 78.2 \\
   % \cline{3-11}
      %& & +\shortdataset{} && \textbf{30.88} & \textbf{36.9} & \textbf{49.8} && \textbf{12.60} & \textbf{58.2} & \textbf{86.6} \\
      & & +\shortdataset{} && \textbf{27.49} & \textbf{36.2} & \textbf{50.5} && \textbf{13.03} & \textbf{57.1} & \textbf{85.1} \\
    \bottomrule
\end{tabular}
}
\caption{Ablation study, evaluating the effect of our progressive training scheme over the two test sets (\cambridge{} in the top rows, and \megadepth{} in the bottom rows). All experiments start with the cropped panoramas used in Cai \emph{et al.}~\cite{cai2021extreme}. Best results are in bold,
and second best are underlined. }
\label{tab:ablation}
\end{table}

==> tables/ablation_auxilary_short.tex <==
\definecolor{graytext}{RGB}{130,130,130}
\begin{table}[t]
\setlength{\tabcolsep}{1.7pt}
% \def\arraystretch{1.05}
 \def\arraystretch{1.02}
%  \footnotesize
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lllccccccccccccccccc} %{0.88\textwidth}
%{p{1.5cm}p{1.5cm}p{1.5cm}lp{1.5cm}p{1.5cm}p{1.5cm}lp{1.5cm}p{1.5cm}p{1.5cm}}
    \toprule
    & & \multicolumn{3}{c}{}&\multicolumn{3}{c}{Top 1} & & \multicolumn{3}{c}{Top 5} \\
     \cline{6-8} \cline{10-12}
     &Overlap & KP & SM &&MGE & RRA$_{15}$ &RRA$_{30}$ && MGE & RRA$_{15}$ & RRA$_{30}$ \\
    \midrule
    % Add your data rows here
    %TODO - instruct w removed scenes
     %\hline
%      \multirow{9}{*}{\rotatebox[origin=c]{90}{\cambridge{}} } & {Large} &  $\times$ & \checkmark && 2.56  & \underline{97.0}  & \underline{97.1}  && 2.59  & \underline{98.6}  & \underline{99.6}  \\
%      & & \checkmark & $\times$ && \underline{2.43}  & \textbf{99.6}  & \textbf{99.7}  && \underline{2.42}  & \textbf{99.7}  & \textbf{100.0}  \\
%    %\cline{3-11}
%    & & \checkmark & \checkmark && \textbf{2.35} & 96.5 & 96.5 && \textbf{2.36} & 96.6 & 96.7 \\
%    %\cline{2-11}
%    &{Small} & $\times$ & \checkmark && \underline{4.42}  & 87.7  &  \underline{90.1} && \underline{4.29}  & \underline{91.9}  & \underline{96.0}  \\
%    && \checkmark & $\times$ && \textbf{4.18}  & \textbf{91.7}  & \textbf{93.6}  && \textbf{4.13}  & \textbf{95.9}  & \textbf{98.9}  \\
%    %\cline{3-11}
%    & & \checkmark & \checkmark && 4.44 & \underline{88.5} & 89.6 && 4.35 & 91.8 & 94.1 \\
%    %\cline{2-11}
%    &{None} & $\times$ & \checkmark && 15.74 & 48.5  & 57.9  && 10.28  & 70.8  & 90.7  \\
%    && \checkmark & $\times$ && \underline{13.53}  &  \textbf{53.5}  & \textbf{63.6}  && \underline{9.26}  & \textbf{77.7}  & \textbf{95.6} \\
%    & & \checkmark & \checkmark && \textbf{13.36} & \underline{52.9} & \underline{59.7} && \textbf{9.17} & \underline{76.6} & \underline{94.5} \\
%    \hline
    
%   \multirow{9}{*}{\rotatebox[origin=c]{90}{\megadepth{} }}
%   & {Large}  & $\times$ & \checkmark && 2.57  & 96.3  & 97.0  && 2.57  & 98.2  & \underline{99.6}  \\
%   %\cline{3-11}
%   && \checkmark & $\times$ && \textbf{2.39} & \textbf{97.7}  & \textbf{98.4} 
%   && \textbf{2.34}  & \underline{98.5}  & \textbf{99.7} \\
%   %\cline{3-11}
%   & & \checkmark & \checkmark && \underline{2.40}  & \textbf{97.7}  & \underline{98.2}  && \underline{2.39}  & \textbf{98.6}  & 99.4 \\
%   %\cline{2-11}
%   &{Small} & $\times$ & \checkmark && 5.57  & 81.4  & 88.8  && 5.28  & 87.1  & 96.0  \\
%   & & \checkmark & $\times$ && \underline{4.75} &\underline{ 84.0}  & \underline{89.4}   && \underline{4.53}  & \underline{89.1}  & \underline{96.5} \\
%   %\cline{3-11}
%   & & \checkmark & \checkmark && \textbf{4.33} & \textbf{88.1} & \textbf{92.3} && \textbf{4.12} & \textbf{91.2} & \textbf{97.1}  \\
%   %\cline{2-11}
%   &{None} & $\times$ & \checkmark && 46.0  & 28.5  & 42.5  && 14.75  & 50.7  & 79.2  \\ 
%   && \checkmark & $\times$ && \underline{42.09} & \underline{33.4}  & \underline{45.9}  
%   && \underline{12.78}  & \underline{56.3}  & \underline{84.0}  \\
%   & & \checkmark & \checkmark &&  \textbf{27.49} & \textbf{36.2} & \textbf{50.5} && \textbf{13.03} & \textbf{57.1} & \textbf{85.1}  \\
%
\ignorethis{
    \multirow{9}{*}{\rotatebox[origin=c]{90}{\cambridge{}} } & {Large} & $\times$ & $\times$ && 2.24  & 92.8  & 93.2  && 2.24  & 98.3  & 98.9  \\ 
    &&  $\times$ & \checkmark && 2.56  & 97.0  & 97.1  && 2.59  & 98.6  & 99.6  \\
      & & \checkmark & $\times$ && 2.43  &  \textbf{99.6}  &  \textbf{99.7}  && 2.42  &  \textbf{99.7}  &  \textbf{100.0}  \\
    %\cline{3-11}
    & & \checkmark & \checkmark &&  \textbf{2.35} & 96.5 & 96.5 &&  \textbf{2.36} & 96.6 & 96.7 \\
    %\cline{2-11}
    &{Small} & $\times$ & $\times$ && 4.31  & 91.7  & 93.3  && 4.28  & 94.8  & 98.2  \\ 
    && $\times$ & \checkmark && 4.42  & 87.7  &  90.1 && 4.29  & 91.9  & 96.0  \\
    && \checkmark & $\times$ &&  \textbf{4.18} &  \textbf{91.7}  &  \textbf{93.6} &&  \textbf{4.13}  &  \textbf{95.9}  &  \textbf{98.9}  \\
    %\cline{3-11}
    & & \checkmark & \checkmark && 4.44 & 88.5 & 89.6 && 4.35 & 91.8 & 94.1 \\
    %\cline{2-11}
    &{None} & $\times$ & $\times$ && 20.44  & 45.0  & 53.1  && 10.05  & 68.5  & 87.2  \\ 
    && $\times$ & \checkmark && 15.74 & 48.5  & 57.9  && 10.28  & 70.8  & 90.7  \\
    && \checkmark & $\times$ && 13.53  &   \textbf{53.5}  &  \textbf{63.6}  && 9.26  &  \textbf{77.7}  &  \textbf{95.6} \\
    & & \checkmark & \checkmark &&  \textbf{13.36} & 52.9 & 59.7 &&  \textbf{9.17} & 76.6 & 94.5 \\
    \hline
    }
    %\multirow{9}{*}{\rotatebox[origin=c]{90}{\megadepth{} }}
    & {Large}  & $\times$ & $\times$ && 2.19  & 96.0  & 96.6  && 2.23  & 98.3  & 99.3  \\ 
    && $\times$ & \checkmark && 2.57  & 96.3  & 97.0  && 2.57  & 98.2  & 99.6  \\
    %\cline{3-11}
    && \checkmark & $\times$ &&  \textbf{2.39} & 97.7  &  \textbf{98.4} 
    &&  \textbf{2.34}  &  98.5  &  \textbf{99.7} \\
    %\cline{3-11}
    & & \checkmark & \checkmark && 2.40  &  \textbf{97.7}  & 98.2  && 2.39 &  \textbf{98.6}  & 99.4 \\
    %\cline{2-11}
    &{Small} & $\times$ & $\times$ && 4.39  & 87.8  & 91.2  && 4.24  & 91.0  & 95.2  \\ 
    && $\times$ & \checkmark && 5.57  & 81.4  & 88.8  && 5.28  & 87.1  & 96.0  \\
    & & \checkmark & $\times$ && 4.75 & 84.0  & 89.4   && 4.53  & 89.1  & 96.5 \\
    %\cline{3-11}
    & & \checkmark & \checkmark &&  \textbf{4.33} &  \textbf{88.1} &  \textbf{92.3} &&  \textbf{4.12} &  \textbf{91.2} &  \textbf{97.1}  \\
    %\cline{2-11}
    &{None} 
    & $\times$ & $\times$ && 49.31  & 33.1  & 44.0  && 12.92  & 56.5  &  \textbf{85.4}  \\ 
    && $\times$ & \checkmark && 46.00  & 28.5  & 42.50  && 14.75  & 50.7  & 79.2  \\ 
    && \checkmark & $\times$ && 42.09 & 33.4  & 45.9  
    && \textbf{12.78}  & 56.3  & 84.0  \\
    & & \checkmark & \checkmark &&   \textbf{27.49} &  \textbf{36.2} &  \textbf{50.5} &&  13.03 &  \textbf{57.1} &  {85.1}  \\
    \bottomrule
\end{tabular}
}
\vspace{-8pt}
\caption{Ablation study, evaluating the effect of the auxiliary channels added as input to our network. We train models without the keypoints and matches (KP) and without the segmentation maps (SM), comparing to our model over the \megadepth{} test set.} %\hec{add two x's} }
\label{tab:auxillary}
\end{table}

==> tables/ablation_ch.tex <==
\definecolor{graytext}{RGB}{130,130,130}
\begin{table}[t]
\setlength{\tabcolsep}{1.7pt}
% \def\arraystretch{1.05}
 \def\arraystretch{1.2}
%  \footnotesize
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lllccccccccccccccccc} %{0.88\textwidth}
%
    \toprule
    & \multicolumn{6}{c}{}&\multicolumn{3}{c}{Top 1} & & \multicolumn{3}{c}{Top 5} \\
     \cline{8-10} \cline{12-14}
     &Overlap && \fovexp{} & \instructexp{} & \shortdataset{} &&MGE & RRA$_{15}$ &RRA$_{30}$ && MGE & RRA$_{15}$ & RRA$_{30}$ \\
    \midrule

      \multirow{15}{*}{\rotatebox[origin=c]{90}{\cambridge{}} } & Large &&   $\times$&$\times$& $\times$&&  8.17 & 86.4 & 97.1 && 8.17 & 87.5 & 98.1\\
      
      & && $\vee$&$\vee$&$\vee$ && 2.91  & \textbf{99.8}  & \textbf{99.8}  && 2.87  & \textbf{99.8}  & \textbf{100.0}  \\

    & && \checkmark&$\times$& $\times$&& 3.18 & 98.2 & 98.2 && 3.21 & 97.9& 98.7 \\

    & &&\checkmark&\checkmark& $\times$ && 3.10 & 99.4 & 99.5 && 4.04 & 98.5 & 98.9\\

    & && \checkmark&\checkmark& \checkmark && \textbf{2.35} & 96.5 & 96.5 && \textbf{2.36} & 96.6 & 96.7  & \vspace{1pt} \\ 

    &Small && $\times$&$\times$& $\times$ && 26.44 & 6.3 & 60.2 && 22.32 & 17.4 & 69.5\\

    & && $\vee$&$\vee$&$\vee$&& 5.87  & \textbf{89.4}  & \textbf{93.2}  && 5.47  & \textbf{93.0}  & \textbf{99.5}  \\

    & && \checkmark&$\times$& $\times$ && 5.14 & 79.8 & 82.6 && 5.24 & 85.5 & 92.1 \\

     & && \checkmark&\checkmark& $\times$ && 5.91 & 83.9 & 88.4 && 5.84 & 88.3 & 95.5 \\

    & && \checkmark&\checkmark& \checkmark && \textbf{4.44} & 88.5 & 89.6 && \textbf{4.35} & 91.8 & 94.1  & \vspace{1pt} \\

    &None && $\times$&$\times$& $\times$ && 76.63 & 17.9 & 32.9 && 17.54 & 42.0 & 78.9 \\

    & && $\vee$&$\vee$&$\vee$&& 16.40  & 47.9  & 59.5  && 10.23  & 70.7  & 93.5  \\

    & && \checkmark&$\times$& $\times$ && 28.22 & 42.4 & 49.7 && 10.52 & 71.0 & 90.8 \\

    & && \checkmark&\checkmark& $\times$ && 14.20 & 50.1 & 60.1 && 9.76 & 72.7 & 92.6 \\

     & && \checkmark&\checkmark& \checkmark && \textbf{13.36} & \textbf{52.9} & \textbf{59.7} && \textbf{9.17} & \textbf{76.6} & \textbf{94.5} \\
     
    \midrule
     \multirow{15}{*}{{\rotatebox[origin=c]{90}\megadepth{}}} & Large && $\times$&$\times$& $\times$ && 13.65 & 35.4 & 73.5 && 12.22 & 61.4 & 84.7\\

     & && $\vee$&$\vee$&$\vee$&& 2.67  & 96.9  & 98.0  && 2.62 & 98.2  & \textbf{99.7}  \\

    & && \checkmark&$\times$& $\times$ && 4.61 & 79.7 & 81.1 && 4.41 & 90.3& 98.9\\

    & && \checkmark&\checkmark& $\times$ && 4.46 & 90.4 & 92.4 && 4.43 & 94.3 & 99.1 \\

    & && \checkmark&\checkmark& \checkmark && \textbf{2.40} & \textbf{97.7} & \textbf{98.2} && \textbf{2.39} & \textbf{98.6} & 99.4 & \vspace{1pt}\\

    &Small&& $\times$&$\times$& $\times$ && 55.28 & 3.7 & 29.1 && 29.83 & 15.0 & 50.3  \\

    & && $\vee$&$\vee$&$\vee$&& 6.35  & 80.9  & 90.0  && 6.09  & 87.1  & \textbf{97.9}  \\

    & && \checkmark&$\times$& $\times$ && 12.91 & 56.2 & 68.2 && 10.97 & 66.0 & 85.4 \\

    & && \checkmark&\checkmark& $\times$ && 11.46 & 62.5 & 80.6 && 10.73 & 68.0 & 91.0 \\

     & && \checkmark&\checkmark& \checkmark && \textbf{4.33} & \textbf{88.1} & \textbf{92.3} && \textbf{4.12} & \textbf{91.2} & 97.1 & \vspace{1pt}\\

    &None && $\times$&$\times$& $\times$ && 74.94 & 12.8 & 25.3 && 25.11 & 26.1 & 58.8  \\

    & && $\vee$&$\vee$&$\vee$ && 66.87  & 26.1  & 36.2  && 15.53  & 47.3  & 75.0  \\

    & && \checkmark&$\times$& $\times$ && 61.62 & 25.0 & 38.4 && 16.82 & 44.2 & 75.0 \\
    & && \checkmark&\checkmark& $\times$ && 68.31 & 25.0 & 36.1 && 16.21 & 45.7 & 78.2 \\
      & && \checkmark&\checkmark& \checkmark && \textbf{27.49} & \textbf{36.2} & \textbf{50.5} && \textbf{13.03} & \textbf{57.1} & \textbf{85.1} \\
    \bottomrule
\end{tabular}
}
\caption{Ablation study, evaluating the effect of our progressive training scheme over the two test sets (\cambridge{} in the top rows, and \megadepth{} in the bottom rows). All experiments start with the cropped panoramas used in Cai \emph{et al.}~\cite{cai2021extreme}. We also assess the necessity of the  progressive training scheme compared to training on all pairs simultaneously. Comparison denoted with $\vee$ is training with all of the datasets together. Best results are in bold. }
\label{tab:ablation_ch}
\end{table}

==> tables/ablation_progressive_short.tex <==
\definecolor{graytext}{RGB}{130,130,130}
\begin{table}[t]
\setlength{\tabcolsep}{1.7pt}
% \def\arraystretch{1.05}
 \def\arraystretch{1.02}
%  \footnotesize
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lllccccccccccccccccc} %{0.88\textwidth}
%{p{1.5cm}p{1.5cm}p{1.5cm}lp{1.5cm}p{1.5cm}p{1.5cm}lp{1.5cm}p{1.5cm}p{1.5cm}}
    \toprule
    & \multicolumn{3}{c}{}&\multicolumn{3}{c}{Top 1} & & \multicolumn{3}{c}{Top 5} \\
     \cline{5-7} \cline{9-11}
     &Overlap & Train data &&MGE & RRA$_{15}$ &RRA$_{30}$ && MGE & RRA$_{15}$ & RRA$_{30}$ \\
    \midrule
    % Add your data rows here
    %TODO - instruct w removed scenes
     %\hline
%    \multirow{12}{*}{\rotatebox[origin=c]{90}{\cambridge{}} } & Large & \cite{cai2021extreme} &&  8.17 & 86.4 & 97.1 && 8.17 & 87.5 & 98.1\\
% % \cline{3-11}
%  & & +\fovexp{} && \underline{3.18} & \underline{98.2} & \underline{98.2} && \underline{3.21} & \underline{97.9}& \underline{98.7} \\
% % \cline{3-11}
%  & & +\instructexp{} && 3.10 & \textbf{99.4} & \textbf{99.5} && 4.04 & \textbf{98.5} & \textbf{98.9} \\
% % \cline{3-11}
%  %& & +\shortdataset{} && \textbf{2.32} & 89.9 & 89.9 && \textbf{2.31} & 89.9 & 90.2  & \vspace{1pt} \\ 
%  & & +\shortdataset{} && \textbf{2.35} & 96.5 & 96.5 && \textbf{2.36} & 96.6 & 96.7  & \vspace{1pt} \\ 
%%  \cline{2-11}
%  &Small & \cite{cai2021extreme} && 26.44 & 6.3 & 60.2 && 22.32 & 17.4 & 69.5\\
%%  \cline{3-11}
%  & & +\fovexp{} && \underline{5.14} & 79.8 & 82.6 && \underline{5.24} & 85.5 & 92.1 \\
% % \cline{3-11}
%   & & +\instructexp{} && 5.91 & \underline{83.9} & \underline{88.4} && 5.84 & \underline{88.3} & \textbf{95.5} \\
% % \cline{3-11}
%  %& & +\shortdataset{} && \textbf{4.53} & \underline{82.8} & \underline{85.5} && \textbf{4.36} & \underline{86.3} & 90.9  & \vspace{1pt} \\
 %   & & +\shortdataset{} && \textbf{4.44} & \textbf{88.5} & \textbf{89.6} && \textbf{4.35} & \textbf{91.8} & \underline{94.1}  & \vspace{1pt} \\
 % %  \cline{2-11}
 %   &None & \cite{cai2021extreme} && 76.63 & 17.9 & 32.9 && 17.54 & 42.0 & 78.9 \\
 % %  \cline{3-11}
 %   & & +\fovexp{} && 28.22 & 42.4 & 49.7 && 10.52 & 71.0 & 90.8 \\
 % %  \cline{3-11}
 %   & & +\instructexp{} && \underline{14.20} & \underline{50.1} & \underline{60.1} && \underline{9.76} & \underline{72.7} & \underline{92.6} \\
 %   %\cline{3-11}
 %    %& & +\shortdataset{} && \textbf{13.29} & \textbf{51.7} & \underline{57.1} && \textbf{9.28} & \textbf{72.8} & 90.2 \\
 %    & & +\shortdataset{} && \textbf{13.36} & \textbf{52.9} & \textbf{59.7} && \textbf{9.17} & \textbf{76.6} & \textbf{94.5} \\
 %   \midrule
 %    \multirow{12}{*}{{\rotatebox[origin=c]{90}\megadepth{}}} & Large & \cite{cai2021extreme} && 13.65 & 35.4 & 73.5 && 12.22 & 61.4 & 84.7\\
 %   %\cline{3-11}
 %   & & +\fovexp{} && 4.61 & 79.7 & 81.1 && \underline{4.41} & 90.3& 98.9\\
 %   %\cline{3-11}
 %   & & +\instructexp{} && \underline{4.46} & \underline{90.4} & \underline{92.4} && 4.43 & \underline{94.3} & \underline{99.1} \\
    %\cline{3-11}
    %& & +\shortdataset{} && \textbf{2.21} & \textbf{97.4} & \textbf{98.2} && \textbf{2.19} & \textbf{98.0} & \textbf{99.1} & \vspace{1pt}\\
%    & & +\shortdataset{} && \textbf{2.40} & \textbf{97.7} & \textbf{98.2} && \textbf{2.39} & \textbf{98.6} & \textbf{99.4} & \vspace{1pt}\\
%    %\cline{2-11}
%    &Small& \cite{cai2021extreme} && 55.28 & 3.7 & 29.1 && 29.83 & 15.0 & 50.3  \\
%    %\cline{3-11}
%    & & +\fovexp{} && 12.91 & 56.2 & 68.2 && 10.97 & 66.0 & 85.4 \\
%   % \cline{3-11}
%    & & +\instructexp{} && \underline{11.46} & \underline{62.5} & \underline{80.6} && \underline{10.73} & \underline{68.0} & \underline{91.0} \\
% %   \cline{3-11}
%     %& & +\shortdataset{} && \textbf{4.69} & \textbf{83.2} & \textbf{89.1} && \textbf{4.59} & \textbf{87.4} & \textbf{96.4} & \vspace{1pt}\\
%     & & +\shortdataset{} && \textbf{4.33} & \textbf{88.1} & \textbf{92.3} && \textbf{4.12} & \textbf{91.2} & \textbf{97.1} & \vspace{1pt}\\
%  %  \cline{2-11}
%    &None & \cite{cai2021extreme} && 74.94 & 12.8 & 25.3 && 25.11 & 26.1 & 58.8  \\
 %   \cline{3-11}
%    & & +\fovexp{} && \underline{61.62} & \underline{25.0} & \underline{38.4} && 16.82 & 44.2 & 75.0 \\
%    %\cline{3-11}
%    & & +\instructexp{} && 68.31 & \underline{25.0} & 36.1 && \underline{16.21} & \underline{45.7} & \underline{78.2} \\
%   % \cline{3-11}
      %& & +\shortdataset{} && \textbf{30.88} & \textbf{36.9} & \textbf{49.8} && \textbf{12.60} & \textbf{58.2} & \textbf{86.6} \\
%      & & +\shortdataset{} && \textbf{27.49} & \textbf{36.2} & \textbf{50.5} && \textbf{13.03} & \textbf{57.1} & \textbf{85.1} \\
\ignorethis{
      \multirow{12}{*}{\rotatebox[origin=c]{90}{\cambridge{}} } & Large & \cite{cai2021extreme} &&  8.17 & 86.4 & 97.1 && 8.17 & 87.5 & 98.1\\
   % \cline{3-11}
    & & +\fovexp{} && 3.18 & 98.2 & 98.2 && 3.21 & 97.9& 98.7 \\
   % \cline{3-11}
    & & +\instructexp{} && 3.10 & \textbf{99.4} & \textbf{99.5} && 4.04 & \textbf{98.5} & \textbf{98.9}\\
   % \cline{3-11}
    %& & +\shortdataset{} && \textbf{2.32} & 89.9 & 89.9 && \textbf{2.31} & 89.9 & 90.2  & \vspace{1pt} \\ 
    
    & & +\shortdataset{} && \textbf{2.35} & 96.5 & 96.5 && \textbf{2.36} & 96.6 & 96.7  & \vspace{1pt} \\ 
  %  \cline{2-11}
    &Small & \cite{cai2021extreme} && 26.44 & 6.3 & 60.2 && 22.32 & 17.4 & 69.5\\
  %  \cline{3-11}
    & & +\fovexp{} && 5.14 & 79.8 & 82.6 && 5.24 & 85.5 & 92.1 \\
   % \cline{3-11}
     & & +\instructexp{} && 5.91 & 83.9 & 88.4 && 5.84 & 88.3 & 95.5 \\
   % \cline{3-11}
    %& & +\shortdataset{} && \textbf{4.53} & \underline{82.8} & \underline{85.5} && \textbf{4.36} & \underline{86.3} & 90.9  & \vspace{1pt} \\
    & & +\shortdataset{} && \textbf{4.44} & \textbf{88.5} & \textbf{89.6} && \textbf{4.35} & \textbf{91.8} & \textbf{94.1}  & \vspace{1pt} \\
  %  \cline{2-11}
    &None & \cite{cai2021extreme} && 76.63 & 17.9 & 32.9 && 17.54 & 42.0 & 78.9 \\
  %  \cline{3-11}
    & & +\fovexp{} && 28.22 & 42.4 & 49.7 && 10.52 & 71.0 & 90.8 \\
  %  \cline{3-11}
    & & +\instructexp{} && 14.20 & 50.1 & 60.1 && 9.76 & 72.7 & 92.6 \\
    %\cline{3-11}
     %& & +\shortdataset{} && \textbf{13.29} & \textbf{51.7} & \underline{57.1} && \textbf{9.28} & \textbf{72.8} & 90.2 \\
     & & +\shortdataset{} && \textbf{13.36} & \textbf{52.9} & \textbf{59.7} && \textbf{9.17} & \textbf{76.6} & \textbf{94.5} \\
    \midrule
    }
      & Large & \cite{cai2021extreme} && 13.65 & 35.4 & 73.5 && 12.22 & 61.4 & 84.7\\
    %\cline{3-11}
    & & +\fovexp{} && 4.61 & 79.7 & 81.1 && 4.41 & 90.3& 98.9\\
    %\cline{3-11}
    & & +\instructexp{} && 4.46 & 90.4 & 92.4 && 4.43 & 94.3 & 99.1 \\
    %\cline{3-11}
    %& & +\shortdataset{} && \textbf{2.21} & \textbf{97.4} & \textbf{98.2} && \textbf{2.19} & \textbf{98.0} & \textbf{99.1} & \vspace{1pt}\\
    & & +\shortdataset{} && \textbf{2.40} & \textbf{97.7} & \textbf{98.2} && \textbf{2.39} & \textbf{98.6} & \textbf{99.4} & \vspace{1pt}\\
    %\cline{2-11}
    &Small& \cite{cai2021extreme} && 55.28 & 3.7 & 29.1 && 29.83 & 15.0 & 50.3  \\
    %\cline{3-11}
    & & +\fovexp{} && 12.91 & 56.2 & 68.2 && 10.97 & 66.0 & 85.4 \\
   % \cline{3-11}
    & & +\instructexp{} && 11.46 & 62.5 & 80.6 && 10.73 & 68.0 & 91.0 \\
 %   \cline{3-11}
     %& & +\shortdataset{} && \textbf{4.69} & \textbf{83.2} & \textbf{89.1} && \textbf{4.59} & \textbf{87.4} & \textbf{96.4} & \vspace{1pt}\\
     & & +\shortdataset{} && \textbf{4.33} & \textbf{88.1} & \textbf{92.3} && \textbf{4.12} & \textbf{91.2} & \textbf{97.1} & \vspace{1pt}\\
  %  \cline{2-11}
    &None & \cite{cai2021extreme} && 74.94 & 12.8 & 25.3 && 25.11 & 26.1 & 58.8  \\
 %   \cline{3-11}
    & & +\fovexp{} && 61.62 & 25.0 & 38.4 && 16.82 & 44.2 & 75.0 \\
    %\cline{3-11}
    & & +\instructexp{} && 68.31 & 25.0 & 36.1 && 16.21 & 45.7 & 78.2 \\
   % \cline{3-11}
      %& & +\shortdataset{} && \textbf{30.88} & \textbf{36.9} & \textbf{49.8} && \textbf{12.60} & \textbf{58.2} & \textbf{86.6} \\
      & & +\shortdataset{} && \textbf{27.49} & \textbf{36.2} & \textbf{50.5} && \textbf{13.03} & \textbf{57.1} & \textbf{85.1} \\
    \bottomrule
\end{tabular}
}
\vspace{-8pt}
\caption{Ablation study, evaluating the effect of our progressive training scheme over the \megadepth{} test set. All experiments start with the cropped panoramas used in Cai \emph{et al.}~\cite{cai2021extreme}. %Best results are in bold,and second best are underlined. 
}
\label{tab:ablation}
\end{table}

==> tables/cascaded_att.tex <==
\definecolor{graytext}{RGB}{130,130,130}
\begin{table}[t]
\setlength{\tabcolsep}{1.7pt}
% \def\arraystretch{1.05}
 \def\arraystretch{1.02}
%  \footnotesize
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lccccccccccccccccc} %{0.88\textwidth}
%{p{1.5cm}p{1.5cm}p{1.5cm}lp{1.5cm}p{1.5cm}p{1.5cm}lp{1.5cm}p{1.5cm}p{1.5cm}}
    \toprule
    && \multicolumn{2}{c}{Large} && \multicolumn{2}{c}{Small} && \multicolumn{2}{c}{None} \\
     \cline{3-4} \cline{6-7} \cline{9-10}
     Method &&MGE & RRA$_{10}$ &&MGE & RRA$_{10}$ &&MGE & RRA$_{10}$ \\
    \midrule

CascadedAtt~\cite{dekel2024estimating} &&   0.48 &  100.0 && 0.72 &  100.0 && 1.20 & 96.2\\
Our Implemetation  &&  1.42 & 100.0 &&  1.89 & 98.3 && 2.06 &  96.2\\
     \bottomrule
\end{tabular}
}
\vspace{-8pt}
\caption{\textbf{Cascaded Attention} Since CascadedAtt~\cite{dekel2024estimating}  model weights were not released, we compare results on the Streetlearn panoramas test set, as reported in ~\cite{dekel2024estimating}, with our implementation described in the baselines section.
}
\label{tab:cascaded_att}
\end{table}

==> tables/dataset-statistics.tex <==


\begin{table}[t]
\setlength{\tabcolsep}{3.8pt}
% \def\arraystretch{1.05}
 \def\arraystretch{0.95}
%  \footnotesize
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{llcccccccccccc}
\toprule & & \multicolumn{4}{c}{\#Pairs} \\ 
\cline{3-7} 
Subset
& Source & \#Scenes &  Large & Small & None & Total  \\ 
\midrule
Train   & \cite{tung2024megascenes}  & 6398 & 40000                   & 15492    & 33657      & 89149                        \\
\cambridge{} & \cite{kendall2015cambridgelandmarks}    & 6 & 2512        & 827      & 1961    & 5300                            \\
\megadepth{}  & \cite{li2018megadepth} & 17 & 2700       & 829                      & 643                  &  4172                          \\

\bottomrule
\end{tabular}
}
\vspace{-8pt}
\caption{\textbf{\dataset{} Dataset Statistics}. Above, we report the number of image pairs extracted for each overlap level, split into train and test (with \cambridge{} denoting a \emph{single} camera setting and \megadepth{} denoting the ``in the \emph{wild}" setting).}
\label{tab:dataset-statistics}
\end{table}





==> tables/main_table.tex <==
\definecolor{graytext}{RGB}{130,130,130}
\begin{table}[t]
\setlength{\tabcolsep}{1.7pt}
% \def\arraystretch{1.05}
 \def\arraystretch{1}
%  \footnotesize
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{llcccccccccc} %{0.88\textwidth}

    \toprule
    \multicolumn{2}{c}{}&&\multicolumn{3}{c}{\cambridge{}}&&
    \multicolumn{3}{c}{\megadepth{}}\\
    \cline{4-6} \cline{8-10}
      & Method &&MGE & RRA$_{15}$ &RRA$_{30}$ && MGE & RRA$_{15}$ & RRA$_{30}$ \\
    \midrule

    \multirow{6}{*}{\rotatebox[origin=c]{90}{Large}} & %SIFT*~\cite{lowe2004distinctive} &&  1.29 & 96.6 & 97.3 &&  %\textbf{ 1.33} & 96.5 & 97.5 \\
    SIFT*~\cite{lowe2004distinctive} && 1.95  & 92.3 & 95.3 && 2.94  & 74.6 & 80.8 \\
    %& LoFTR*~\cite{sun2021loftr} &&   1.69 & 92.2 & 94.7 &&   2.43 & 84.8 & 90.9 \\
    & LoFTR*~\cite{sun2021loftr} &&   1.76 & 97.2 & 99.1 &&  2.13  & 85.2 & 93.8 \\
    & DenseCorrVol~\cite{cai2021extreme} &&   98.51 & 25.9 & 33.3 &&   120.53 & 7.0 & 13.0 \\   &CascadedAtt~\cite{dekel2024estimating}&&   29.75 & 42.7 & 50.0 && 170.62 & 7.3 & 9.2\\
        & 8PointViT~\cite{rockwell20228} &&   22.33 & 31.9 & 64.8 && -- & -- & -- \\
    & 
    Dust3R~\cite{wang2023dust3r} &&  \textbf{0.77} & \textbf{99.7} & \textbf{99.9} &&    \colorbox{lightgray}{1.01} &  \colorbox{lightgray}{98.4} &  \colorbox{lightgray}{99.2} \\
    % & Mast3R~\cite{leroy2024groundingimagematching3d} &&  {1.00} & \textbf{99.8} & {99.6} &&    \colorbox{lightgray}{1.35} &  \colorbox{lightgray}{99.0} &  \colorbox{lightgray}{99.6} \\

    & Ours&&   2.35 & 96.5 & 96.5 &&   \textbf{2.40} & \textbf{97.7} & \textbf{98.2} \\
    \midrule
    \multirow{6}{*}{\rotatebox[origin=c]{90}{Small}} & %SIFT$^*$~\cite{lowe2004distinctive} &&   \textcolor{gray}{1.90} & \textcolor{gray}{84.8} & \textcolor{gray}{88.3} &&   4.24 & 81.1 & 88.7 \\
    SIFT*~\cite{lowe2004distinctive} && 5.07  & 64.7 & 71.3 && \textcolor{gray}{7.27}  & \textcolor{gray}{61.4} & \textcolor{gray}{68.4} \\
    %& LoFTR$^*$~\cite{sun2021loftr} &&   \textcolor{gray}{24.04} & \textcolor{gray}{42.2} & \textcolor{gray}{54.9} &&   \textcolor{gray}{29.20} & \textcolor{gray}{30.1} & \textcolor{gray}{52.1 }\\
    & LoFTR$^*$~\cite{sun2021loftr} &&   \textcolor{gray}{2.70} & \textcolor{gray}{81.5} & \textcolor{gray}{93.6} &&   \textcolor{gray}{6.80} & \textcolor{gray}{66.6} & \textcolor{gray}{81.2 }\\
    & DenseCorrVol~\cite{cai2021extreme} &&   143.47 & 2.8 & 9.4 &&   125.73 & 3.1 & 9.4 \\
   &CascadedAtt~\cite{dekel2024estimating}&&   148.44 & 0.0 & 3.0 && 139.14 & 2.7 & 4.4\\
        & 8PointViT~\cite{rockwell20228}  &&   51.30 & 1.7 & 12.8 && -- & -- & --\\
    & Dust3R~\cite{wang2023dust3r} &&   \textbf{1.96} & \textbf{95.9} & \textbf{94.6} && \colorbox{lightgray}{{2.80}} & \colorbox{lightgray}{{89.8}} & \colorbox{lightgray}{{94.4}}\\
    % & Mast3R~\cite{leroy2024groundingimagematching3d} &&  2.13 & 90.9 & 93.9 &&    \colorbox{lightgray}{3.47} &  \colorbox{lightgray}{91.6} &  \colorbox{lightgray}{96.7} \\
    & Ours &&   4.44 & 88.5 & 89.6 &&  \textbf{4.33} & \textbf{88.1} & \textbf{92.3} \\
    \midrule
    \multirow{6}{*}{\rotatebox[origin=c]{90}{None}} & %SIFT*~\cite{lowe2004distinctive} &&    \textcolor{gray}{130.33} &   \textcolor{gray}{0.0} &  \textcolor{gray}{0.0} &&    \textcolor{gray}{120.96} &  \textcolor{gray}{9.5} &  \textcolor{gray}{14.3} \\
    SIFT*~\cite{lowe2004distinctive} && \textcolor{gray}{121.94}  & \textcolor{gray}{2.7} & \textcolor{gray}{5.4} && \textcolor{gray}{122.84}  & \textcolor{gray}{0.0} & \textcolor{gray}{2.0} \\
    %& LoFTR*~\cite{sun2021loftr} &&  \textcolor{gray}{ 157.72 }& \textcolor{gray}{ 0.0 }& \textcolor{gray}{2.6 }&& \textcolor{gray}{ 56.22 }& \textcolor{gray}{5.9 }& \textcolor{gray}{29.4} \\
    & LoFTR*~\cite{sun2021loftr} &&  \textcolor{gray}{ - }& \textcolor{gray}{ - }& \textcolor{gray}{- }&& \textcolor{gray}{ 56.54 }& \textcolor{gray}{0.0 }& \textcolor{gray}{33.0} \\
    & DenseCorrVol~\cite{cai2021extreme} && 77.10 & 9.0 & 27.0 &&   82.04 & 2.9 & 13.7 \\
%&8PointViT~\cite{rockwell20228}  &&   123.03 & 0.0 & 0. && - & - & -\\
% 8PointViT~\cite{rockwell20228}  &&   -- & -- & -- && -- & -- & --\\
    &CascadedAtt~\cite{dekel2024estimating}&&   69.69 & 8.4 & 23.1 && 78.60 & 7.5 & 20.8 \\
    & Dust3R~\cite{wang2023dust3r} &&   114.33 & 19.8 & 23.9 && \colorbox{lightgray}{{81.21}} & \colorbox{lightgray}{{15.4}} & \colorbox{lightgray}{{26.9}}\\
    % & Mast3R~\cite{leroy2024groundingimagematching3d} &&    {18.85} & {42.8} & \textbf{60.5} &&    \colorbox{lightgray}{55.93} &  \colorbox{lightgray}{22.0} &  \colorbox{lightgray}{37.9} \\
    & Ours &&   \textbf{13.36} & \textbf{52.9} & \textbf{59.7} &&   \textbf{27.49} & \textbf{36.2} & \textbf{50.5} \\
    \bottomrule
\end{tabular}
}
\vspace{-8pt}
\caption{\textbf{Rotation Estimation in the Wild.} We evaluate performance over the \cambridge{} and \megadepth{} test sets, separately considering Large (top), Small (middle) and Non-overlapping (bottom) pairs. 
%We report the mean and median geodesic error in degrees, and the percentage of pairs with a relative rotation error under 10$^\circ$ for different levels of overlap. %Models trained only on overlapping pairs are denoted with ``-o''. 
$^*$ indicates median errors are computed only over successful image pairs, for which these algorithms output a pose estimate (failure over more than $50\%$ of the test pairs is shown in gray). 
\colorbox{lightgray}{Note that Dust3R was trained on images from \megadepth{}.}
}

\label{tab:main_result}
\end{table}


